Reinforcement Learning for Neural Model Editing

Editing pretrained neural networks requires specialized algorithms tailored to specific objectives. Designing such algorithms is often time-consuming and demands significant effort. We present an exploratory framework that formulates neural model editing as a reinforcement learning problem, where agents modify models using only reward feedback. We introduce two environments: MaskWorld, where agents scale weights multiplicatively, and ShiftWorld, where agents apply additive weight updates. The reward function combines a utility-preservation objective with a task-specific editing objective, enabling agents to learn targeted modifications while maintaining overall model performance. We evaluate the framework on bias mitigation in text classification and machine unlearning in image classification, both of which traditionally rely on specialized algorithms. Our results show that the learned edits reduce forget set accuracy to 0% while preserving over 90% retain set accuracy in the unlearning setting. In the bias mitigation setting, the learned edits improve performance on an unbiased evaluation dataset by more than 7% while maintaining general classification utility. These findings suggest that reinforcement learning can serve as a general framework for learning neural model editing policies from reward feedback.

==> latex/5_conclusion.tex <==
\section{Conclusion}
\begin{comment}
That's actually a much stronger and more honest framing for this kind of paper. It positions HyperRL as an **exploratory framework paper** rather than a benchmark-chasing one, which suits the work better given that the RL agent is genuinely doing something structurally different from existing approaches.

The story you want to tell is something like:

> *Gradient-based model editing works well when you can define a differentiable loss. But many desirable model behaviors — fairness, unlearning, spurious correlation removal — are most naturally expressed as reward signals, not loss functions. We ask: can a single, unified RL framework serve as a flexible substrate for all of these goals, requiring only a reward function to be specified?*

This framing has several advantages for ACL reviewers:

- It sidesteps the "why not just use gradient ascent" objection by acknowledging gradient methods work fine *when applicable*, and positioning RL as complementary rather than competing
- It makes the two-task demonstration (unlearning + bias mitigation) read as **proof of flexibility** rather than an incomplete benchmark comparison
- It naturally motivates future work — the framework is the contribution, and future papers can plug in new reward functions for new goals
- It's intellectually honest about the current results, which show the method *works* rather than *dominates*

The related works section I drafted leans a little too hard toward "and HyperRL beats all of these." Want me to revise it to better reflect this framing — motivating the *field of inquiry* and emphasizing the framework's flexibility and generality over any competitive comparison?
\end{comment}

